D-Brane Systems in Twisted Holography and SO/Sp Chiral Algebras

We study correlation functions of baryon and determinant operators for the chiral algebras obtained from the twist of N = 4 SYM with U(N) gauge group. In the context of Twisted Holography, we conjecture that a dual description should involve a D1-D5 brane system, and we construct from the correlators a candidate dual brane in the form of a derived coherent sheaf in SL(2,C). Extending this analysis, we compute similar baryon/determinant correlators of chiral algebras in symmetric and antisymmetric representations of SO and Sp gauge groups and construct the candidate dual branes. These branes exhibit Z_2 identifications consistent with conjectures relating SO/Sp chiral algebras to Kodaira-Spencer theory on SL(2,C)/Z_2 and the Type I topological string on SL(2,C).

==> 2_A_Complex_for_an_Instanton/subsections/1_review_of_determinants_and_saddles.tex <==
The basic determinant operators we make use of in this work take the form

\begin{equation}
	\det \left(m + Z(z;u) \right) \qquad\text{with} \qquad Z(z;u)=X(z) + u Y(z)
\end{equation}

Insertions of these correspond in the large N limit to the presence of probe D1-branes. This may be argued heuristically from a 't Hooft expansion perspective by writing the determinant as an integral:

\begin{align}\label{eq:fermionized_determinant}
	\int d \bar \psi d \psi e^{\bar \psi \left(m + Z \right)\psi}
\end{align}

with auxiliary fermionic degrees of freedom $\psi$ and $\psibar$ which, being in the fundamental and anti-fundamental representation of the gauge group, provide worldsheet boundaries in a large $N$ ribbon graph expansion.

This correspondence was made precise in \cite{giant_gravitons_kasia}, where they were able to map a correlation function of determinant operators to a 2d surface in $SL_2(\bC)$ i.e. the corresponding dual brane. 

The first step in their construction uses techniques developed in pedagogical detail by \cite{Komatsu_2020}, that allow to recast expectation values of determinant operators as integrals over auxiliary matrix degrees of freedom which are then amenable to a saddle point analysis. 

Summarizing quickly \cite{Komatsu_2020}'s procedure, one first writes the determinants as fermionic integrals as in \eqref{eq:fermionized_determinant} and integrates out the $X$ and $Y$ fields:

\begin{align}
\prod_\alpha \det \left(m_\alpha + Z(z_\alpha;u_\alpha) \right) &= \int d \bar \psi d \psi \,e^{\sum_\alpha \bar \psi^\alpha \left(m_\alpha + Z(z_\alpha;u_\alpha) \right)\psi_\alpha }\,\\
&= \int d \bar \psi d \psi e^{-\frac{1}{N} \sum_{\alpha<\beta} \frac{u_\alpha-u_\beta}{z_\alpha - z_\beta}\bar \psi^\beta\psi_\alpha \, \bar \psi^\alpha\psi_\beta}
\end{align}

One then ``factorizes" the quartic $\psi$ interaction as one mediated by a cubic interaction through an auxiliary field matrix $\rho$:

\begin{align}
\prod_\alpha &\det \left(m_\alpha + Z(z_\alpha; u_\alpha) \right) = \\
&\left[\prod_{\alpha < \beta} \frac{1}{2 \pi i } \frac{u_\alpha-u_\beta}{z_\alpha - z_\beta}\right]\int d \bar \psi d \psi d \rho\,  e^{N \sum_{\alpha<\beta} \frac{z_\alpha - z_\beta}{u_\alpha-u_\beta} \rho^\alpha_\beta \rho^\beta_\alpha + \sum_{\alpha\neq \beta} \rho^\alpha_\beta \bar \psi^\beta\psi_\alpha }
\end{align}

and finally, one integrates out the fermions:

\begin{align}\label{eq:integrate_out_psis}
\prod_\alpha &\det \left(m_\alpha + X(z_\alpha) + u_\alpha Y(z_\alpha) \right) = \\
&\left[\prod_{\alpha < \beta}\frac{1}{2 \pi i } \frac{u_\alpha-u_\beta}{z_\alpha - z_\beta}\right]\int  d \rho \, e^{N \log \rho + N \sum_{\alpha<\beta} \frac{z_\alpha - z_\beta}{u_\alpha-u_\beta} \rho^\alpha_\beta \rho^\beta_\alpha}
\end{align}

Performing a saddle point analysis in the large N limit, we find this last integral is dominated by $\rho$'s which satisfy the saddle equation:

\begin{equation}\label{eq:U(N)_saddle_eq}
(u_\alpha-u_\beta) (\rho^{-1})^\alpha_\beta + (z_\alpha - z_\beta) \rho^\alpha_\beta =0 
\end{equation}

which may be expressed as a matrix equation:

\begin{equation}\label{eq:U(N)_saddle_eq}
[\zeta,\rho] + [\mu,\rho^{-1}] = 0
\end{equation}

in terms of the diagonal matrices: 

\begin{equation}\label{eq:saddle_eq}
\mu^\alpha_\beta = u_\alpha \delta^\alpha_\beta \qquad \text{and} \qquad \zeta^\alpha_\beta = z_\alpha \delta^\alpha_\beta
\end{equation}


==> 2_A_Complex_for_an_Instanton/subsections/2_a_brane_as_a_spectral_curve.tex <==
The holographic dictionary proposed by \cite{giant_gravitons_kasia} identifies the $\rho$ saddle with a D-brane supported on the spectral curve for the commuting matrices 
\begin{align}\label{eq:B,C,D}
B(a) &= \mu a - \rho \cr
C(a) &= \zeta a + \rho^{-1} \cr
D(a) &= \frac{1+CB}{a} = \frac{1+BC}{a}\\
&= \mu \zeta a - \zeta \rho +  \rho^{-1} \mu = \mu \zeta a - \rho \zeta +  \mu \rho^{-1} 
\end{align}

which satisfy $a\,D(a) - B(a)C(a) = 1$. \al{Maybe provide a justification for this definition} In other words, we consider the one-complex-dimensional spaces of quadruples $(a,b,c,d)$ where $b$, $c$, $d$ are eigenvalues of the above matrices with a common eigenvector. 

==> 2_A_Complex_for_an_Instanton/subsections/3_a_brane_as_a_complex.tex <==
The previous presentation obfuscates a bit the $SL(2)_L \times SL(2)_R$ symmetries of the problem \al{I have to define them more explicitly if I use this sentence}, simply because it gives the $a$ coordinate a preferential treatment. It is one of the main results of this work to provide a construction that respects these symmetries.

To do so let's rewrite the condition that the $B,C,D$ matrices have a common eigenvector as the statement that the set of matrices 
\begin{align}
B(a)-b &= \mu a -b - \rho \cr
C(a)-c &= \zeta a -c + \rho^{-1} \cr
D(a)-d &= \mu \zeta a -d - \zeta \rho + \rho^{-1} \mu 
\end{align}

have a common null vector. If we multiply the second matrix by $\mu$ on the right and subtract it from the third we get a more symmetric pair of matrices 
\begin{align}\label{eq:new_matrices}
M_1 &\coloneqq \mu a -b - \rho \cr
M_2 &\coloneqq \mu c -d - \zeta \rho 
\end{align}
which are co-variant under $SL(2)_L \times SL(2)_R$ and have a common null vector on the spectral curve. Had we used the equivalent expression for $D(a) = \mu \zeta a - \rho \zeta  + \mu \rho^{-1} $, and instead multiplied $C-c$ with $\mu$ from the left, we would've obtained the matrix 
\begin{align}
M_2' \coloneqq \mu c -d - \rho \zeta
\end{align}

We'll make use of $M_2'$ momentarily.

Conversely, if $M_1$ and $M_2$ have a common null vector then we must have common eigenvector for $B$ by definition of $M_1$ and $C$ since 
\begin{equation}	
cM_1 - aM_2  = c(\mu a -b - \rho ) - a(\mu c -d - \zeta \rho) = ( \zeta a -c + \rho^{-1})\rho =(C(a)-c)\rho
\end{equation}

So we conclude that the $B,C,D$ matrices have a common eigenvector iff  $M_1$ and $M_2$  have a common null vector with the latter giving a more symmetric presentation of the spectral curve. 

Finally, a D-brane in the B-model is not uniquely characterized by its support: that information should be supplemented by a line bundle or vector bundle on the worldvolume. 
A candidate line bundle was guessed in \cite{giant_gravitons_kasia}, however a better way to present a D-brane is as a complex of coherent sheaves which we proceed to do. 

Denote as $l$ the number of determinant insertions. There is a reasonably standard way to build a complex for a spectral curve \al{Maybe write down the complex in terms of $B$ and $C$, and say the following is quasi-isomorphic}:  
\begin{equation}\label{eq:brane_complex}
\bC^{l} \xrightarrow{d_1} \bC^{l} \oplus \bC^{l} \xrightarrow{d_2} \bC^{l}
\end{equation}

with maps $d_1$ and $d_2$ given in terms of the $M_1$, $M_2$ and $M_2'$ matrices \al{WRONG COMPLEX CHECK YOUR IPAD}
\begin{align}
d_1 &= {-\rho^{-1} M_2'\choose  \,\,\,\,\,\rho^{-1}M_1} \\
d_2 &= \left(M_1 \quad  M_2\right) 
\end{align}

explicitly
\begin{align}\label{eq:brane_differentials}
d_1 &= {-\rho^{-1}(\mu c - d) + \zeta \choose \,\,\,\,\,\rho^{-1}(\mu a -b) - 1}\\
d_2 &= \left(\mu a - b -\rho \quad \mu c -d -\zeta\rho\right)
\end{align}

and condition $d_2 d_1=0$ guaranteed by the fact that $\rho$ is a saddle
\begin{align}
d_2 d_1 = M_1\rho^{-1}M_2' - M_2 \rho^{-1} M_1 = [\zeta, \rho]+ [\mu, \rho^{-1}]
\end{align}

The complex is a very natural candidate to define the D1 brane dual to a given saddle. \al{Are there any checks needed?}


% The condition that $B,C$, and therefore $D$, were mutually commuting was guaranteed by virtue of $\rho$ being a saddle
% \begin{align}
% [B(a),C(a)] = a([\zeta, \rho]+ [\mu, \rho^{-1}])
% \end{align}

% One may find a third equivalent statement in terms of $M_1, M_2$ and $M_2'$ by substituting $B$ and $C$ in the expression above:
% \begin{align}
% M_1 \rho^{-1} M_2' - M_2 \rho^{-1} M_1 = [\zeta, \rho]+ [\mu, \rho^{-1}]
% \end{align}


==> 2_A_Complex_for_an_Instanton/subsections/4_with_fundamentals_come_baryons.tex <==

Our chiral algebras admit interesting modifications where we add fundamental fields $J$ and anti-fundamentals $I$ with action:

\begin{align}
\int \dd^2z \, I\bar\partial J
\end{align}

The classical BRST transformations act on $I$ and $J$ by gauge transformations with parameter $c$. This translates into an extra term in the BRST charge $\pm\oint\Tr IcJ$ which may spoil nilpotency of $Q_{\text{BRST}}$ quantum mechanically. 
In order to cancel such anomalies, we need to add both bosonic and fermionic fields in equal number. We denote the number of fundamental fields of each type as $F$ so that the resulting chiral algebra classically has $U(F|F)$ global symmetry. When necessary, we can denote individual components as $J^i_A$ and $I^A_j$ with $A,B$ the $U(F|F)$ flavor indices and  $i,j$ gauge indices.
It is a bit tedious to keep track of signs from Grassmann parity so to lighten expressions we will treat the $I$ and $J$ fields as if they were Grassmann odd. 

Another point of convention is how to normalize the $IJ$ OPE. The choice is pretty immaterial \al{Maybe add $\hbar$}.  
\begin{equation}
	J^a_A(z) I^B_b(w) \sim %\textcolor{red}{\frac{1}{N}?}
 \frac{\delta^a_b \delta^B_A}{z-w}\,.
\end{equation}

% The BRST current now has an extra $\Tr c J I$ term. The tree-level BRST charge acts on $I$ and $J$ by gauge transformations with parameter $c$. 

% The currents for the $U(F|F)$ symmetry are just $j^A_B \equiv I^A J_B$. They are $Q$-closed in the $SU(N)$ theory. In a $U(N)$ theory they would have an anomaly forcing them to be traceless and the diagonal current would be $Q$-exact. 

% This sort of anomaly affects the mesonic operators 
% \begin{equation}
% 	E^A_B(u;z) \equiv  I^A (X + u Y)^n J_B
% \end{equation}
% These are $Q$-closed at tree level, but at 1-loop we can contract $I$ and $J$ to get something like $\delta^A_B \Tr \partial c (X + u Y)^n$. Furthermore,
% $Q_0 \Tr b (X + u Y)^n = N^{-1} E^A_A(u;z)$. Hence only the traceless part of the mesons is $Q$-closed and the meson proportional to $\delta^A_B$ can be rewritten in terms of traces \al{To do: elaborate further upon this so I can see more crisply which operators are Q-closed and which fail to be}. 

% The action of $Q$ on operators built from $X$ and $Y$ is unaffected by the extra flavours, so that correlation functions of 
% $A_n$'s or determinant operators are unchanged. 

There is a great deal of holographic information that can be extracted from these \al{COMPLETE}  Holographically, the presence of flavours is expected to correspond to
the presence of space-filling branes in the bulk. The brane created by standard determinant operators could simply be superimposed to these 
 without any effect. 
 
The combined set of branes, though, admits novel deformations akin to the ones which can deform a 
D0-D4 system to a collection of instantons on the D4 brane world-volume. We expect these to map to 
modifications of determinant operators involving the $I$ and $J$ fields. Our objective in this section is to establish a dictionary between such modifications
 \al{in the planar limit?} and a candidate bulk instanton. 

These modifications will be a mixture of the determinant operators of the previous section and baryonic operators such as 
\begin{equation}
\label{eq:baryonic}
\varepsilon_{i_1 \cdots i_N} J^{i_1}_{A_1} \cdots J^{i_n}_{A_n}
\end{equation}

However, for these to be Q-closed, we'll need for our chiral algebra to have $SU(N)$ and not $U(N)$ gauge group. A few remarks about this new chiral algebra are in order.

The new OPE in the $SU(N)$ theory is modified to 
\begin{equation}
	Y^a_b(z) X^c_d(w) \sim \left[\frac{\delta^a_d \delta^c_b}{N}-\frac{\delta^a_b \delta^c_d}{N^2}\right]\frac{1}{z-w}
\end{equation}
Gauge invariant functions of $Z(z;u)=X(z)+uY(z)$ are still Q-closed as the reasoning used in the $U(N)$ case still holds. Our determinant operators fall into this category.  However, their correlation functions acquire subleading corrections
\begin{align}
	\Biggl<\prod_i &\det \left(m_i + Z(z_i;u_i)\right) \Biggr> = \cr &= \int d \bar \psi d \psi e^{-\frac{1}{N} \sum_{i<j} \frac{u_i-u_j}{z_i - z_j}\bar \psi_j\psi^i \, \bar \psi_i\psi^j-\frac{1}{N^2} \sum_{i<j} \frac{u_i-u_j}{z_i - z_j}\bar \psi_j\psi^j \, \bar \psi_i\psi^i + \sum_i m_i\psibar_i\psi^i }%:\,e^{\sum_i \bar \psi^i \left(m_i + X(z_i) + u_i Y(z_i) \right)\psi_i }\,:
\end{align}
We can account for that by acting with  
\begin{equation}
	e^{-\frac{1}{N^2} \sum_{i<j} \frac{u_i-u_j}{z_i - z_j}\partial_{m_i} \partial_{m_j}}
\end{equation}
\al{Is there a physical interpretation for this expression? It seems like one is wick contracting m's as if they were a field themselves} but this gives a change of order $1$ and does not affect the semi-classical saddle. \al{check details of this}

Returning to the baryons, we can fermionize them as 
\begin{equation}
\varepsilon_{i_1 \cdots i_N} J^{i_1}_{A_1} \cdots J^{i_n}_{A_n} = \int d \bar \psi e^{\bar \psi J \epsilon}
\end{equation}
where $\epsilon^A$ are parameters. We can similarly fermionize an anti-baryon:
\begin{equation}
	\int d\psi e^{ \bar \epsilon I \psi}
\end{equation}
with parameters $\bar \epsilon_A$. 

For example, the correlation function of a baryon and an anti-baryon is 
\begin{equation}
	\left\langle \int d \bar \psi d\psi  e^{ \bar \psi J(z) \epsilon+\bar \epsilon I(w) \psi}\right\rangle =\int d \bar \psi d\psi  e^{\frac{1}{z-w}  \bar \epsilon \epsilon \bar \psi \psi} 
\end{equation}

We can try to combine a baryon and an anti-baryon at the same point: 
\begin{equation}
	\int d \bar \psi d \psi e^{\bar \psi J \epsilon+\bar \epsilon I \psi}
\end{equation}
but there is a 1-loop anomaly proportional to $\bar \epsilon \epsilon$. We can cancel by requiring $\bar \epsilon \epsilon =0$.

Such an operator can be expanded into a polynomial in $IJ$ currents, in the same way as a determinant can be expanded into traces. 
We can also deform it to
\begin{equation}
	\int d \bar \psi d \psi e^{m \bar \psi \psi + \bar \psi J \epsilon+\bar \epsilon I \psi} = m^N e^{\frac{\bar \epsilon IJ \epsilon}{m}}
\end{equation}
More interestingly, we can consider
\begin{equation}
	\mathcal{O}(m,z,u,\epsilon,\bar\epsilon) \coloneqq\int d \bar \psi d \psi e^{\bar \psi \left(m + X(z) + u Y(z) \right)\psi+ \bar \psi J \epsilon+\bar \epsilon I \psi}
\end{equation}
interpolating between a determinant and a product of a baryon and an anti-baryon. We need again  $\bar \epsilon \epsilon =0$ in order to avoid an anomaly. These are natural candidates to describe a deformation of the bulk brane system. 



==> 2_A_Complex_for_an_Instanton/subsections/5_The_Instanton_Complex.tex <==

The expectation value of normal ordered products of such operators can be computed as before. The contractions between $I$'s and $J$'s will now contribute the extra terms: 
\begin{equation}
	\bra\prod_i \mathcal{O}_i\ket = \int[\dd\psibar][\dd\psi]  e^{\cdots \,+ \sum_{i\neq j} \frac{1}{z_i-z_j}   \epsilon^i \bar\epsilon_j \psibar_i  \psi^j }
\end{equation}
one then may perform the same Hubbard-Stratonovich transformation and integrate out the $\psibar \psi$'s

\begin{equation}
	\bra\prod_i \mathcal{O}_i\ket = \frac{1}{Z_\rho}\int [\dd\rho ]\exp\left(\frac{N}{2}\sum_{i\neq j}\frac{z_i - z_j}{u_i - u_j}\rho^i_j\rho^j_i + N\Tr\left(\ln \left(\rho + \frac{1}{z-z}\epsilon\bar\epsilon\right)\right)\right)\\
\end{equation}
which after a shift $\rho^i_j \mapsto \rho^i_j - \frac{1}{z_i - z_j} \epsilon^i\bar\epsilon_j$, leads to a modified saddle equation:
\begin{equation}
(z_i - z_j)\rho^i_j + (u_i- u_j)(\rho^{-1})^i_j  = \epsilon^i\bar\epsilon_j \quad \text{equivalently} \quad [\zeta,\rho] + [\mu, \rho^{-1}] = \epsilon\bar\epsilon
 \label{eq:SEflavour}
\end{equation}

with $\zeta$ and $\mu$ the same diagonal matrices with eigenvalues $z_i$ and $u_i$ respectively. Note these equations may only hold if the BRST condition $\epsilon^i\bar\epsilon_i$=0 is satisfied.

If we write as before 
\begin{align}
B(a) &= a \mu -  \rho\\
C(a) &= a \zeta + \rho^{-1} 
\end{align}
then $B$ and $C$ no longer commute. Instead, they satisfy 
\begin{equation}
	[B(a), C(a)] = a \epsilon\bar\epsilon
\end{equation}
which resembles the F-term constraints on the data of an ADHM construction of an instanton configuration. 

The corresponding ADHM  construction would use a complex of the form 
\begin{equation}
	\bC^f \xrightarrow{d_1} \bC^{f} \oplus \bC^{f} \oplus \bC^{F|F} \xrightarrow{d_2} \bC^f
\end{equation}

with maps $d_1$ and $d_2$ which satisfy $d_2 d_1=0$. We find that the natural choice extending \eqref{eq:brane_complex} and \eqref{eq:brane_differentials}
\begin{align}
d_1 &= 
\begin{pmatrix}
-\rho^{-1}(\mu c - d) + \zeta \\
\,\,\,\,\,\rho^{-1}(\mu a -b) - 1\\
-\bar\epsilon
\end{pmatrix}\\
d_2 &= \left(\mu a - b -\rho \quad \mu c -d -\zeta\rho \quad \epsilon\right)
\end{align}
gives precisely such a complex.

We therefore propose this as our candidate D-brane system \al{instanton somewhere?} holographic dual to a specific saddle for the correlation function of generalized determinants. 
{\bf How can we test this proposal? Can we compute the variation of an action? Single trace 1-pt functions?}
